WAVER: Writing-style Agnostic Text-Video Retrieval via Distilling Vision-Language Models Through Open-Vocabulary Knowledge

Text-video retrieval, a prominent sub-field within the domain of multimodal information retrieval, has witnessed remarkable growth in recent years. However, existing methods assume video scenes are consistent with unbiased descriptions. These limitations fail to align with real-world scenarios since descriptions can be influenced by annotator biases, diverse writing styles, and varying textual perspectives. To overcome the aforementioned problems, we introduce $\texttt{WAVER}$, a cross-domain knowledge distillation framework via vision-language models through open-vocabulary knowledge designed to tackle the challenge of handling different writing styles in video descriptions. $\texttt{WAVER}$ capitalizes on the open-vocabulary properties that lie in pre-trained vision-language models and employs an implicit knowledge distillation approach to transfer text-based knowledge from a teacher model to a vision-based student. Empirical studies conducted across four standard benchmark datasets, encompassing various settings, provide compelling evidence that $\texttt{WAVER}$ can achieve state-of-the-art performance in text-video retrieval task while handling writing-style variations. The code is available at: https://github.com/Fsoft-AIC/WAVER

==> sections/Rebuttal.tex <==
=================Reviewer #352E=================
We sincerely thank the reviewer for dedicating their time to carefully review our work and for providing valuable feedback, particularly acknowledging the well-motivated and thoroughly evaluated of our research.

=================Reviewer #4EA1=================
We appreciate the reviewer's comments on the knowledge distillation (KD) mechanism and our significance and innovation.

We apologize for any confusion that may have arisen regarding the reviewer's concerns about "offering only incremental advancements" and the perception that "KD mechanisms to address this task are not new to our community." We would like to clarify as follows:

Firstly, we want to emphasize that our work tackles a novel problem in text-video retrieval, referred as "writing-style agnostic," which has not been addressed in existing literature. This challenge, prevalent in NLP, is a common occurrence in text-video retrieval, yet none of the existing works have effectively tackled it.

Secondly, our inclusion of KD in the related work section was intended to highlight its status as an existing technique. We fully acknowledge that KD itself is not our contribution. However, the novelty arises from our innovative utilization of KD to address the "writing-style agnostic" aspect in text-video retrieval. This is a unique approach that has not been explored previously.

Thirdly, we conducted extensive experiments across four major datasets (Tables 1-4) and performed various ablation studies (Tables 5-8) to showcase the significance and innovation of our proposed WAVER. Our results clearly demonstrate substantial performance gains over the runner-up method across multiple metrics. These experiments and analyses serve as strong evidence of the significant contributions our work makes to the field.

In summary, we firmly assert that WAVER presents a novel framework designed to address the unique challenge of "writing-style agnostic" in Text-Video Retrieval. Our approach harnesses a cross-domain knowledge distillation (KD) mechanism that leverages open-vocabulary properties to effectively utilize the potent representation knowledge obtained from pre-trained vision-language models. This innovative approach underscores the distinct and valuable contribution of our work.

=================Reviewer #488A=================
We sincerely thank the reviewer for their valuable time and feedback, which acknowledge the effectiveness of our WAVER employing a cross-domain knowledge distillation mechanism to address writing-style variations. We appreciate the recognition of WAVER's superior performance in text–video retrieval tasks. We take into account the reviewer's valuable suggestions regarding figure descriptions and citing "Distilling the Knowledge in a Neural Network." We will ensure that figure descriptions are added in the final version, and we'll also incorporate the recommended citation. 






==> sections/Rebuttal_2.tex <==
**Reviewer #352E**
We genuinely value the reviewer's dedication of time and expertise in carefully assessing our work. We are grateful for their recognition of our well-motivated research and thorough evaluation.

**Reviewer #4EA1**

We thank the reviewer's comments and would like to address the concerns as follows:

- Our paper does not intend to propose a new knowledge-distillation (KD) mechanism. Instead, our inclusion of KD in the Related Work section was intended to highlight its status as an existing technique. Our novelty lies in utilizing KD innovatively to tackle the "writing-style agnostic" problem. We believe that the problem we address as well as the proposed framework in this study has not yet been studied in existing literature.

- The "writing-style agnostic" problem arises from manual annotations by different annotators, resulting in imperfect annotations, diverse writing styles, and varying perspectives. This issue is common in text-video retrieval, but previous works have not effectively addressed it. Our proposal is the first to tackle this challenge.

- In our Related Work section, we emphasize that prior KD studies primarily revolve around teacher-student models for knowledge transfer. In contrast, our model extracts knowledge from open-vocabulary phrases, encompassing a wide range of writing styles. This approach sets our framework apart, as it uses open-vocabulary knowledge implicitly as a teacher to transfer substantial knowledge for text-video retrieval.

- To substantiate the significant contributions of our work to the field, we conducted extensive experiments across four major datasets (Tables 1-4) and performed various ablation studies (Tables 5-8) to showcase the significance and innovation of our proposed WAVER. Our results clearly demonstrate substantial performance gains over the runner-up method across multiple metrics.

- In summary, our contribution lies in the innovative use of KD to address the "writing-style agnostic" problem, without proposing a new KD mechanism. Additionally, our unique approach involves utilizing open-vocabulary knowledge as an implicit teacher for knowledge transfer in text-video retrieval.

**Reviewer #488A**

We sincerely thank the reviewer for their valuable time and feedback, which acknowledge the effectiveness of our WAVER employing a cross-domain knowledge distillation mechanism to address writing-style variations. We appreciate the recognition of WAVER's superior performance in text–video retrieval tasks. We take into account the reviewer's valuable suggestions regarding figure descriptions and citing "Distilling the Knowledge in a Neural Network." We ensure that the figure's detailed descriptions will be added in the final version, and we will also incorporate the recommended citation. 


